Decoder Gradient Shield: Provable and High-Fidelity Prevention of Gradient-Based Box-Free Watermark Removal

The intellectual property of deep image-to-image models can be protected by the so-called box-free watermarking. It uses an encoder and a decoder, respectively, to embed into and extract from the model's output images invisible copyright marks. Prior works have improved watermark robustness, focusing on the design of better watermark encoders. In this paper, we reveal an overlooked vulnerability of the unprotected watermark decoder which is jointly trained with the encoder and can be exploited to train a watermark removal network. To defend against such an attack, we propose the decoder gradient shield (DGS) as a protection layer in the decoder API to prevent gradient-based watermark removal with a closed-form solution. The fundamental idea is inspired by the classical adversarial attack, but is utilized for the first time as a defensive mechanism in the box-free model watermarking. We then demonstrate that DGS can reorient and rescale the gradient directions of watermarked queries and stop the watermark remover's training loss from converging to the level without DGS, while retaining decoder output image quality. Experimental results verify the effectiveness of proposed method. Code of paper will be made available upon acceptance.

==> sec_abandoned/0_abstract.tex <==
\begin{abstract}
% The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
% Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
% The abstract is to be in 10-point, single-spaced type.
% Leave two blank lines after the Abstract, then begin the main text.
% Look at previous \confName abstracts to get a feel for style and length.
The intellectual property of deep image-to-image models can be protected by the so-called box-free watermarking, which involves an encoder and a decoder, respectively, to embed into and extract from the model output images invisible copyright marks. Prior works have improved watermark robustness focusing on the design of better watermark encoders. However, in this paper, we reveal the overlooked vulnerability of the unprotected watermark decoder which is jointly trained with the encoder and can be exploited to train a watermark removal network. To fill this gap, we propose the decoder gradient shield (DGS), serving as a protection layer in the decoder API, to prevent gradient-based watermark removal. Specifically, DGS reorients the gradient directions of watermarked queries and can stop the watermark remover training loss from converging to the level without DGS, while this is achieved with the preservation of decoder output image quality and with the efficient $\mathcal{O}\left(1\right)$ time complexity. The proposed method is inspired by the classic adversarial attack, while it is for the first time utilized as a defensive mechanism in box-free model watermarking. Both theoretical derivations and experimental results are provided to verify the effectiveness of the proposed method. Code of the paper is available upon acceptance.
\end{abstract}

==> sec_abandoned/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% Since the introduction of AlexNet \cite{}, neural networks have rapidly gained momentum. Landmark models such as ResNet \cite{}, YOLO \cite{}, and Transformer \cite{} have demonstrated exceptional performance, often surpassing human capabilities in various tasks. However, these resource-intensive models face the risk of intellectual property infringement, posing threats of misuse, data privacy breaches, and hindrances to innovation. To address these challenges, model watermarking techniques have been employed to verify the ownership and detect model theft.
Today's deep learning models can provide exceptional performance across a wide range of tasks, even surpassing human capability. However, these resource-intensive models are facing the risk of intellectual property infringement. To address this problem, model watermarking has been developed to verify model ownership or detect model theft.

% Model watermarking can be broadly classified into three categories based on how the watermark is extracted. White-box methods require access to the model's internal information, such as parameters and feature map \cite{}, for precise watermark embedding and extraction. However, these methods risk privacy leakage and protocol infringement. Black-box methods, also referred to as backdoor watermarking, alter the model's performance when a special input, known as a trigger, is provided, causing the watermark to appear at the model's output \cite{}.
According to how the watermark is extracted, model watermarking can be classified into white-box, black-box, and box-free methods. White-box methods \cite{uchida2017embedding,wang2022rethinking,Lv2023A} require access to the protected model's internal content in which the watermark is encoded. Black-box methods \cite{adi2018turning,Li2023Universal,hua23unambiguous}, also known as backdoor watermarking, require querying the protected model for watermark extraction since they encoder the watermark into the model's input-output mapping. Box-free methods, however, extract the watermark directly from the protected model's outputs, which are more flexible and are specially suitable for models that generate high-entropic content, e.g., encoder-decoder image models \cite{wu2020watermarking,zhang2021deep,zhang2024robust} and generative adversarial networks (GANs) \cite{Lin2024A,Fei2024Wide}. Box-free watermarking is thus also an active method to address the emerging need for AI-generated content attribution. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{figure/victim_architecture1.pdf}
    \caption{Flowchart of box-free model watermarking for image-to-image models. The thin black arrows represent the black-box querying flow (processing and watermarking), while the thick colored arrows represent potential watermark extraction, and each colored arrow pair corresponds to a single input-output pair for $\mathbb{D}$.}
    \label{fig:victim_architecture}
\end{figure}

% Both white-box and black-box methods require access to the protected models (differing in whether internal information is needed) to extract watermarks. In contrast, box-free model watermarking offers greater flexibility by enabling watermark extraction solely from the model’s output, making it a plug-and-play technique. The general workflow of box-free model watermarking is demonstrated in Figure \ref{fig:victim_architecture}, using the protection of an image processing model as an example.
The typical workflow of box-free watermarking for image-to-image models is depicted in Figure \ref{fig:victim_architecture} \cite{zhang2021deep}. Consider a model $\mathbb{M}$ which takes an input $X_0 \in \mathcal{X}_0$ and generates an output $X \in \mathcal{X}$, box-free watermarking creates a watermark encoder $\mathbb{E}$ which embeds a copyright mark image $W$ into $X$ and yield the watermarked image $Y\in\mathcal{Y}$. A dedicated watermark decoder $\mathbb{D}$ is jointly created and can extract the mark $W$ from the watermarked set $\mathcal{Y}$ or a null-mark $W_0$ from the non-watermarked complement set $\mathcal{Y}^\complement$. According to the specific image task, $(\mathcal{X}_0, \mathcal{X})$ can be e.g., (noisy, denoised), (original style, transferred style), etc. In the above process, the model $\mathbb{M}$ is protected by only providing $Y$, instead of $X$, to the user. It has been verified that if the attacker uses the collection of $X_0$ and $Y$ to train a surrogate model, $W$ can still be extracted by $\mathbb{D}$ from the surrogate output images \cite{zhang2021deep}. We refer to $\mathbb{M}$ as either the protected model or the victim model, depending on the context in this paper.

% The protected model $\mathbb{M}$ maps an original image $X_0$ (e.g., a noisy image) to a processed image $X$ (e.g., a denoised image), with both $X_0$ and $X$ accessible to users without protection. Previous research has shown that exposing both $X_0$ and $X$ enables attackers to train a surrogate model that closely replicates $\mathbb{M}$, leading to intellectual property infringement. Box-free model watermarking addresses this by concatenating $X$ with a watermark image $W$ and feeding them into the watermark encoder (embedding network) $\mathbb{E}$, producing the processed and watermarked output $Y$ (also known as the container image). Crucially, $\mathbb{M}$ and $\mathbb{E}$ are encapsulated within a black box, denoted by $\mathbb{B}$, meaning the processed image $X$ is inaccessible to users. As a result, if a surrogate model is trained using the pairs of $X_0$ and $Y$, the watermark will be embedded in its output. The watermark decoder (extraction network) $\mathbb{D}$, which is jointly trained with the encoder $\mathbb{E}$, can accept any input but only extracts the watermark $W$ when $Y$ is provided. For all other inputs, it outputs a blank image $W_0$, indicating the absence of a watermark. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{figure/gradient_based_attack.pdf}
    \caption{Flowchart of gradient-based removal attack. The gradient backpropagated from $\mathbb{D}$ can be estimated leveraging black-box adversarial attacks. In our setting, however, we assume the attacker can directly obtain the gradient without estimation.}
    \label{fig:gradient_based_attack}
\end{figure}

% Existing studies have improved the robustness of box-free model watermarking against basic image processing attacks such as compression, noise addition, and image cropping \cite{<DEBONE_PAMI2>}. However, they overlooked the need for a specific protection mechanism for watermark decoder $\mathbb{D}$. Since $\mathbb{D}$ and $\mathbb{E}$ are jointly trained, they are inherently coupled, meaning $\mathbb{D}$ contains information about $\mathbb{E}$. Without a protection mechanism for $\mathbb{D}$, this coupling could expose information about $\mathbb{E}$, indirectly enabling watermark removal. Specifically, current research assumes that an attacker has black-box access to $\mathbb{D}$, allowing them to obtain input-output pairs. By exploiting this input-output relationship, the attacker can train a watermark remover network $\mathbb{R}$ that estimates the gradients\footnote{Gradient information can be estimated by repeated querying, as demonstrated in black-box adversarial attack literature \cite{}} of $\mathbb{D}$ to remove the watermark from $Y$ while preserving image quality \cite{}.
The attacker has the freedom to alter $Y$ with the hope of removing the watermark while preserving image quality, prior to surrogate training. Intuitively, the alteration can be compression, noise addition, flipping, cropping, etc. Although this vulnerability can be mitigated by adding an augmentation layer between $Y$ and $\mathbb{D}$ when training $\mathbb{E}$ and $\mathbb{D}$ \cite{zhang2024robust}, the attacker can launch a more advanced removal attack by training a removal network $\mathbb{R}$, as shown in Figure \ref{fig:gradient_based_attack}. Adversarial attack literature has proven that the gradient of $\mathbb{D}$ can be estimated via black-box queries, and the gradient can then be used to train $\mathbb{R}$. Such a gradient-based attack is feasible because $\mathbb{D}$ is jointly trained with $\mathbb{E}$ and contains the watermarking mechanism that can be compensated.

% In this paper, we propose a protection scheme for the watermark decoder $\mathbb{D}$, called Gradient Sign Poisoning (GSP), designed to defend against gradient-based watermark removal attacks. In details, ...
In this paper, we first show that the above gradient-based attack can remove state-of-the-art box-free watermarks. Then, under the practical threat model with the gradient information of $\mathbb{D}$ assumed observable to the attacker, we propose a more advanced defense method called decoder gradient shield (DGS). For non-watermarked queries, the black-box API of $\mathbb{D}$ returns the null watermark output (all-white image $W_0$) to the users. For watermarked queries, DGS reorients the corresponding gradient directions so that when the gradient is backpropagated and used to train $\mathbb{R}$, the training loss will not be able to converge to the level without DGS protection. Such reorientation is realized by adding specially crafted perturbations on the output of $\mathbb{D}$, and this is achieved with the preservation of output image quality. We derive the closed-form solution for the proposed perturbation and it enjoys an efficient $\mathcal{O}\left(1\right)$ time complexity. Our contributions are summarized as follows.

\begin{itemize}
\item We reveal that the unprotected watermark decoder in existing box-free watermarking methods can be exploited via black-box access to train a watermark removal network that can remove existing box-free watermarks.

\item We propose the novel DGS with $\mathcal{O}\left(1\right)$ time complexity to \emph{prevent} model extraction exploiting the watermark decoder. This is different from the existing \emph{post-hoc} methods that extract watermarks from successful surrogates.

\item We provide both the close-form derivation and extensive experimental results to verify and demonstrate the effectiveness of the proposed method.
\end{itemize}


% Contribution section may not be a must in a paper.
% Our contributions are summarized as follows
% \begin{itemize}
%     \item 
%     \item 
%     \item 
% \end{itemize}




==> sec_abandoned/2_related_work.tex <==
\section{Related Work}
\label{sec:related work}
\subsection{Model Extraction}
Model extraction, also known as model stealing or surrogate attack, aims to replicate a victim model's functionality, in which the attacker curates a set of query data, and with the victim model returned query outputs, trains a surrogate model. Previous research has mainly focused on stealing deep classification models, in which the surrogate query data can be public data \cite{Orekondy2019Knockoff}, evolutionary proxy data \cite{Barbalau2020Black}, or even synthetic noise \cite{Truong2021Data,Kariyappa2021Maze}, and the attack can be successful even if the victim model only returns hard labels \cite{Sanyal2022Towards}. Model extraction can also be launched against self-supervised image encoder \cite{Sha2023Cant} and ensemble models \cite{Ma2023DivTheft}.

\subsection{Box-Free Watermarking}
Box-free watermarking is named because the watermark is extracted from the model outputs using a dedicated watermark decoder, not requiring the protected model. The watermark decoder can be (1) pretrained and frozen when fine-tuning the protected model for watermark embedding \cite{Lin2024A,Fei2024Wide}, (2) jointly trained with the protected model \cite{wu2020watermarking,Lukas2023PTW}, or (3) a post-hoc model not coupled with the protected model \cite{zhang2021deep,zhang2024robust}. Since the watermarks are embedded in the protected model outputs, box-free methods are commonly applied to generative models with high entropic image outputs.

\subsection{Watermark Removal}
Watermark removal in the context of box-free watermarking is similar yet different from conventional image watermarking. Through the alteration of victim model returned outputs before surrogate training, the removal attack aims to ensure that the watermark cannot be extracted from surrogate model generated images. Such alteration can be either normal image augmentation \cite{zhang2021deep} or a specially designed process such as inpainting \cite{liu2023erase} or an image-to-image watermark remover. These removers are also constrained to preserve the image quality for effective surrogate training.

\subsection{Gradient Attack and Defense}
The attack on neural network gradient has been researched for a decade and is mainly for generating adversarial examples. It can be a white-box attack such as the classic fast gradient sign method (FGSM) \cite{Goodfellow2014Explaining} and projected gradient descent (PGD) \cite{madry2018towards}. Under the more practical black-box setting, the to-be-attacked gradient can be estimated via querying \cite{Ilyas2018Black}, while the required query times can be substantially reduced \cite{Dong2022Query}. These results serve as the foundation of our threat model assuming observable gradient of the black-box decoder to the attacker. In model watermarking, gradient alteration has instead been utilized as a defense approach to protect the extraction of classification models \cite{Mantas2022How}, but it cannot withstand hard-label based extraction \cite{Sanyal2022Towards}. We note that our work is the first to incorporate gradient alteration for protecting image-to-image models. 


==> sec_abandoned/3_problem_formulation.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}
\subsection{Box-free Model Watermarking}
\label{sec:basic}
Since all box-free watermarking methods share the same extraction process using $\mathbb{D}$, without loss of generality, we consider the post-hoc type \cite{zhang2021deep,zhang2024robust} as our watermarking model, whose workflow is depicted in Figure \ref{fig:victim_architecture}. It contains

\begin{itemize}
\item Image Processing: $X \triangleq \mathbb{M}(X_0)$,

\item Watermark Embedding: $Y \triangleq \mathbb{E}({\rm{Concat}}(X, W))$,

\item Watermark Extraction: $\mathbb{D} (\mathcal{Y}) = W$ and $\mathbb{D} (\mathcal{Y}^\complement) = W_0$,
\end{itemize}
where ${\rm{Concat}}(\cdot)$ denotes channel-wise concatenation and $\mathcal{X}_0,\mathcal{X} \subset \mathcal{Y}^\complement$. With $\mathbb{M}$ untouched, $\mathbb{E}$ and $\mathbb{D}$ are jointly trained by minimizing
% This process is designed to satisfy three key requirements: 1) The watermark needs to be successfully embedded and extracted; 2) For images without a watermark, the decoder $\mathbb{D}$ should output an all-white image $W_0$, indicating the absence of a watermark; and 3) The original image-to-image task should remain unaffected, with the watermark being imperceptible to the user (i.e., $Y$ should closely resemble $X$). These requirements are achieved via minimizing the following loss function
\begin{equation}
    \label{eq:loss_joint}
    \mathcal{L}_{\text{Victim}} = \alpha_1 \mathcal{L}_{\text{Embed}} + \alpha_2 \mathcal{L}_{\text{Fidelity}},
\end{equation}
where $\alpha_1$ and $\alpha_2$ are weighting parameters,
\begin{align}
    \mathcal{L}_{\text{Embed}} & = \sum_{Y \in \mathcal{Y}}\|\mathbb{D} \left(Y \right) - W \|_2^2 +  \sum_{S \in \mathcal{Y}^\complement}\|\mathbb{D} \left(S \right) - W_0 \|_2^2, \label{eq:loss_robust}\\
    \mathcal{L}_{\text{Fidelity}} & = \sum_{Y \in \mathcal{Y}, X \in \mathcal{X}} \|Y - X \|_2^2,  \label{eq:loss_fidelity}
\end{align}
and $S$ denotes an arbitrary image. Note that $\mathbb{E}$ is indirectly expressed by its output $Y$ in (\ref{eq:loss_robust}) and (\ref{eq:loss_fidelity}), and this facilitates our subsequent attack formulation in which $\mathbb{E}$ is inaccessible.

\subsection{Threat Model}
% In this paper, two opposing parties are considered: the \textbf{model owner (defender)}, who has invested significant resources in training the model, and the \textbf{malicious user (attacker)}, who seeks to steal the well-trained model for profit.
\textbf{Defender}. We consider the owner of $\mathbb{M}$ as the defender, who not only trains $\mathbb{M}$ but also implements box-free watermarking and owns $\mathbb{E}$ and $\mathbb{D}$. The defender aims to extract watermarks in surrogate model generated images or prevent surrogate training, i.e., incurring non-negligible performance degradation in surrogate models. As shown in Figure \ref{fig:victim_architecture}, the defender only provides the black-box API which accepts query $X_0$ and only returns $Y$, while $\mathbb{M}$ and $\mathbb{E}$ are strictly private. The black-box API of $\mathbb{D}$ is also provided to accept watermark verification queries.

\textbf{Attacker.} On the other side, the attacker aims to extract $\mathbb{M}$ with a watermark-removed surrogate model. To achieve so, the attacker curates a set of $X_0$ to query the victim model and obtains a set of $Y$, which is identical to how normal users behave. Then, prior to surrogate training, the attacker alters $Y$ for watermark removal while preserving image quality. Meanwhile, the attacker can query $\mathbb{D}$ to check if an image contains the defender-embedded watermark. In addition, We assume that the attacker can observe the gradient backpropagated from the output of $\mathbb{D}$, thanks to the adversarial attack literature. Furthermore, the attacker can make a reasonable guess of the existence of potential defender-imposed gradient perturbations if the removal-loss-minimized remover still cannot remove the watermark and can modify the returned gradient as a countermeasure.

% to identify stolen models by ensuring that the embedded watermark remains intact or, if the watermark is removed, that the performance of the surrogate model is significantly inferior to the original.

% \textbf{Defender's Capabilities:} The defender has access to the user's input, as well as the internal details of the model, including its architecture, parameters, and the choice of watermark embedding and extraction schemes.

% \textbf{Attacker's Goal:} 
% The attacker aims to train a surrogate model using the input-output pairs of the victim model without embedded watermarks. To achieve this, they must remove any potential watermark hidden in $Y$.

% \textbf{Attacker's Capabilities:}
% The attacker behaves like a normal user, querying the black-box ($\mathbb{M}$ cascaded with $\mathbb{E}$) and obtaining pairs of $X$ and $Y$. Additionally, the attacker can query the black-box decoder $\mathbb{D}$ for ownership verification using any input, subsequently obtaining the output of $\mathbb{D}$. In essence, the attacker can manipulate $X$, corresponding $Y$, and the input, output of $\mathbb{D}$ in attempts to remove any embedded watermarks.


\subsection{Gradient-based Removal Attack}
We now formulate the gradient-based box-free watermark removal attack depicted in Figure \ref{fig:gradient_based_attack}.
% The rationale behind this attack is the fact that the decoder $\mathbb{D}$ represents the reverse process of the encoder $\mathbb{E}$ and can be exploited to reveal and then revert the watermark embedding mechanism.
The rationale behind is that the attacker can deploy an inverse of $\mathbb{E}$, i.e., another image-to-image network $\mathbb{R}$, which takes in $Y$ and undoes watermark embedding. This can be achieved by using $\mathbb{D}$ as a watermark verifier and an all-white null watermark $W_0$ as the supervision signal, which leads to minimizing
\begin{equation}
\label{eq:loss_attacker}
\mathcal{L}_\text{Attack} = \beta_1 \mathcal{L}_\text{Removal} + \beta_2 \mathcal{L}_\text{Fidelity}^{\text{A}},
\end{equation}
where $\beta_1$ and $\beta_2$ are weighting parameters,
\begin{align}
\mathcal{L}_\text{Removal} & =  \|\mathbb{D}[\mathbb{R}(Y)] - W_0\|_2^2, \label{eq:r_loss}\\
\mathcal{L}_\text{Fidelity}^{\text{A}} & = \|\mathbb{R}(Y) - Y\|_2^2 \label{eq:a_fidelity_loss}. 
\end{align}
The removal loss ensures the altered $Y$, i.e., $\mathbb{R}(Y)$, does not contain the watermark, while the fidelity loss ensures preserved image quality for subsequent surrogate training. To minimize (\ref{eq:r_loss}), it holds that 
\begin{equation}\label{eq:attack_gradient}
\nabla {\mathcal{L}_{{\text{Removal}}}} \propto \frac{{\partial {\mathcal{L}_{{\text{Removal}}}}}}{{\partial \mathbb{D}\left[ {\mathbb{R}(Y)} \right]}}\frac{{\partial \mathbb{D}\left[ {\mathbb{R}(Y)} \right]}}{{\partial \mathbb{R}(Y)}},
\end{equation}
where $\nabla {\mathcal{L}_{{\text{Removal}}}}$ is the gradient component backpropagated to update $\mathbb{R}$ parameters. The $\ell_2$-norm loss function is used in (\ref{eq:r_loss}), while other loss functions can also be used. Under our threat model, the gradient of $\mathbb{D}$ in  (\ref{eq:attack_gradient}), ${\partial \mathbb{D}\left[ {\mathbb{R}(Y)} \right]}/{\partial \mathbb{R}(Y)}$, is observable, and all other gradient components are determined (known) by the attacker. Therefore, $\mathbb{R}$ can be effectively trained in the black-box setting. 

We note that the above attack resembles the classic adaptive filter for model inversion \cite{Haykin2002Adaptive} where $\mathbb{R}$ is an inverse of $\mathbb{E}$. Given the black-box access of $\mathbb{D}$ and without protection, this attack has a theoretical guarantee of convergence.

% One type of removal attack, which is based on gradient estimation, is shown in Figure \ref{fig:gradient_based_attack}. In this attack, the attacker trains a watermark remover network $\mathbb{R}$ to remove the watermark embedded in $Y$ without significant degradation in image quality, modeled as
% \begin{equation}
%     \label{eq:remover_goal}
%     \mathbb{R} \left( Y\right) \approx X.
% \end{equation}

% The above attack requires querying $\mathbb{D}$, whose output can be poisoned in the API before being returned to the users, so that $\mathcal{L}_\text{R}$ cannot be minimized. 





==> sec_abandoned/4_proposed_defense.tex <==
\section{The Proposed Decoder Gradient Shield}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=.85\linewidth]{figure/dgs_architecture.pdf}
    \caption{Flowchart of the proposed DGS in the black-box API of $\mathbb{D}$, where image deraining is used as an example.
    % A conditional branch distinguishes the output derived from watermarked and watermark-free inputs of $\mathbb{D}$. The core transformation is given by $Z^\ast = -PZ + (P+I)W$, where $P$ is a predefined positive definite matrix and $I$ is the identity matrix.
    }
    \label{fig:gsp_architecture}
\end{figure*}
\label{sec:proposed_defense}
The black-box setting of $\mathbb{D}$ enables the defender to alter its output before returning to the user for protection purposes, while the alteration is subject to the constraint of not affecting the watermark extraction functionality. This is similar to API poisoning based defense for black-box (backdoor) watermarking \cite{Zhang2023Categorical}, while it is formulated herein for box-free watermarking. The proposed DGS is derived as follows.

\subsection{Gradient Reorientation}
\label{sec:gr}
For the ease of notation, let $Z \triangleq \mathbb{D}[\mathbb{R}(Y)]$ (see Figure \ref{fig:gradient_based_attack}) and let $Z^{\ast}$ be the altered output that is returned to the user. According to (\ref{eq:r_loss}) and (\ref{eq:attack_gradient}), we have
\begin{equation}
\nabla {\mathcal{L}_{{\text{Removal}}}} \propto  \frac{{\partial {\mathcal{L}_{\text{Removal}}}}}{{\partial \mathbb{R}(Y)}} = 2{\left( Z - {W_0} \right)^T}\frac{\partial Z}{{\partial \mathbb{R}(Y)}},\label{eq:original_gradient}
\end{equation}
where $\{\cdot\}^T$ is the transpose operator. The training of $\mathbb{R}$ requires the curation of a set of $Y$ obtained from querying the encapsulated $\mathbb{M}$ and $\mathbb{E}$ using a set of $X_0$. During the initial training stage, $\mathbb{R}$ is not able to remove the watermark, yielding $Z \approx W$.
% Therefore, the poisoning defense can be decomposed into two goals, i.e., gradient inversion and output quality preservation. Denote the poisoned output by $Z^\ast$ and poisoned gradient by
To prevent $Z$ from eventually converging to $W_0$, we can reorient $Z$ into $Z^\ast$ when $Z \approx W$, so the true gradient direction can be protected. According to (\ref{eq:original_gradient}), the perturbed gradient component can be expressed as 
\begin{equation}
\left(\frac{\partial {\mathcal{L}_{\text{Removal}}}}{\partial \mathbb{R}(Y)}\right)^\ast = 2{\left( {Z^\ast - {W_0}} \right)^T}\frac{{\partial Z^\ast}}{{\partial \mathbb{R}(Y)}}, \label{eq:poison_gradient}
\end{equation}
% then the gradient inversion can be achieved by flipping the sign of (\ref{eq:original_gradient}) in (\ref{eq:poison_gradient}), i.e.,
which can be designed in a way such that the direction change is between $90$ and $180$ degree, i.e.,
\begin{align}
& {\left( {Z^\ast - {W_0}} \right)^T}\frac{{\partial {Z^\ast}}}{{\partial \mathbb{R}(Y)}} = - {\left( {Z - {W_0}} \right)^T}P\frac{{\partial Z}}{{\partial \mathbb{R}(Y)}} \notag\\
\Rightarrow & {\left( {Z^\ast - {W_0}} \right)^T}\frac{{\partial Z^\ast}}{{\partial Z}}= - {\left( {Z - {W_0}} \right)^T}P,\label{eq:z_inverse}
\end{align}
where the chain rule is applied to cancel $\partial Z / \partial \mathbb{R}(Y)$ and $P$ is a positive definite matrix. Note that if $P$ is an identity matrix $I$, then the above reorientation is simply gradient sign flipping ($180$ degree). Meanwhile, to preserve the output image quality, it is required that
\begin{equation}
Z^\ast \approx Z \approx W. \label{eq:z_quality}
\end{equation}
According to (\ref{eq:z_inverse}), the solution for $Z^\ast$ can have the form of
\begin{equation}
Z^\ast = -P Z + C,\label{eq:z_form}
\end{equation}
where $C$ is independent of $Z$. To solve for $C$, substitute (\ref{eq:z_form}) into (\ref{eq:z_quality}), then we have
\begin{equation}
-P Z + C \approx W \Rightarrow C \approx (P+I)W,
\end{equation}
and thus 
\begin{equation}
\label{eq:ultimate_trans}
Z^\ast = -PZ + (P+I)W,
\end{equation}
where the approximation is replaced by equality for implementation. The gradient reorientation in (\ref{eq:ultimate_trans}) is the essential component in the proposed DGS.


\subsection{DGS Protected Decoder API}
We now describe how the proposed gradient reorientation is incorporated in the API of decoder $\mathbb{D}$, as depicted in Figure \ref{fig:gsp_architecture}. Since $\mathbb{D}$ serves as a black-box watermark verifier to end users, we first discuss possible situations of its query denoted by $S$ without deploying the DGS.

\textbf{Situation 1:} $S = Y = \mathbb{E}({\rm{Concat}}(\mathbb{M}(X_0), W)) \in \mathcal{Y}$. This means that $S$ is a processed and watermarked image from the black-box API of $\mathbb{M}$ and it corresponds to the benign query for watermark extraction. It then follows from Section \ref{sec:basic} that it returns $\mathbb{D}(Y) = W$. 

\textbf{Situation 2:} $S = \mathbb{R}(Y)$. This is the malicious query for gradient-based removal attack, but it is indistinguishable from \textbf{Situation 1} because (\ref{eq:a_fidelity_loss}) ensures that $\mathbb{R}(Y)$ is semantically identical to $Y$. However, since the true gradient has not been returned for $\mathbb{R}$ to learn watermark removal, the initial malicious query follows that $S=\mathbb{R}(Y)\in\mathcal{Y}$, and according to Section \ref{sec:gr}, it returns $Z = \mathbb{D}[\mathbb{R}(Y)] = W$.

\textbf{Situation 3:} $S \in \mathcal{Y}^\complement$. This corresponds to the benign query with a non-watermarked image, and it follows from Section \ref{sec:basic} that $\mathbb{D} (\mathcal{Y}^\complement) = W_0$ is returned.

According to the above situations and incorporating (\ref{eq:ultimate_trans}), we can summarize the response mechanism of the DGS protected $\mathbb{D}$ API, denoted by $\mathbb{D}^\ast(S)$, as follows
\begin{equation}\label{eq:final_mechanism}
\mathbb{D}^\ast(S) = \left\{ {\begin{array}{*{20}{l}}
  { - P\mathbb{D}(S) + (P + I)W,}&{{\text{if }}\mathbb{D}(S) \approx W,} \\ 
  {W_0,}&{{\text{otherwise,}}} 
\end{array}} \right.
\end{equation}
meaning that for \textbf{Situations 1} and \textbf{2}, since they are indistinguishable, the API returns the gradient reoriented output, while for \textbf{Situation 3}, the API simply returns the original output. Note that the gradient reorientation in (\ref{eq:final_mechanism}) only adds imperceptible perturbations on the extracted watermark $W$, which does not affect watermark verification, so its influence on normal users is negligible. However, such perturbation can effectively prevent the attacker from training $\mathbb{R}$.


% The gradient reorientation derived in the previous subsection is conditioned on querying $\mathbb{D}$ using watermarked images, i.e., $Y\in\mathcal{Y}$.

% However, (\ref{eq:ultimate_trans}) leads to watermark decoder $\mathbb{D}$ outputting patterns close to the $W$, regardless of whether the input contains a watermark, which contradicts (\ref{eq:loss_robust}), as it requires $\mathbb{D}$ to output a blank image when watermark-free inputs are provided.

% To fill this gap, a conditional branch for $Z$ is introduced. For any input to $\mathbb{D}$, if $Z$ is, or is close to, the blank image $W_0$, it is directly output to the user. Otherwise, if $Z$ is, or is close to, $W$, the transformation in (\ref{eq:ultimate_trans}) will be applied to poison the gradient when training watermark remover $\mathbb{R}$. To sum up, the complete structure of our proposed GSP is illustrated in Figure \ref{fig:gsp_architecture}.

\subsection{Choice of $P$}
\label{sec:p_choice}
The introduced positive definite matrix $P$ can be expressed as
\begin{equation}
\label{matrix_p}
    \begin{bmatrix}
p_{11} & 0 & \cdots & 0 \\
0 & p_{22} & \cdots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
0 & 0 & \cdots & p_{nn}
\end{bmatrix},
\end{equation}
where $n$ is the dimension and $p_{ii} > 0$, $i$ from $1$ to $n$. We clarify its necessity in enhancing the security level of the proposed DGS, even if the defensive scheme is detected by the attacker. We define three degrees of vulnerability.

\textbf{Vulnerability Level 1:} The attacker fails to recognize the existing defensive measures and trains the gradient-based remover accordingly.

\textbf{Vulnerability Level 2:} The attacker acknowledges the existence of the defense but does not understand its mechanism.

\textbf{Vulnerability Level 3:} The attacker detects the reorientation applied to the gradient and takes action.

Vulnerability Level 1 is likely to occur, as the attacker’s observations of the loss curve follow a logical trend, as discussed in Section \ref{sec:convergence_r_loss}. Vulnerability Level 2 is comprehensively discussed in Section \ref{sec:robustness}. The worst-case scenario arises when the attacker detects clues regarding the reoriented gradient, indicating Vulnerability Level 3. A straightforward response for the attacker would be to flip the sign during the updating of remover parameters (e.g., $w_i$), altering the update from
\begin{equation}
    \label{eq:params_update}
    w_i - \frac{\partial \mathcal{L}_{\text{Removal}}}{\partial w_i}
\end{equation}
to
\begin{equation}
    \label{eq:flip_params_update}
    w_i + \frac{\partial \mathcal{L}_{\text{Removal}}}{\partial w_i}
\end{equation}
thus re-reorienting the gradient sign and successfully bypassing the gradient shield if matrix $P$ is not implemented. 

To resolve Vulnerability Level 2, $P$ needs to be introduced with small diagonal elements. We clarify the necessity of this by considering a 2-dimensional example. Based on (\ref{eq:z_inverse}), the key components forming our DGS can be expressed as
\begin{equation}
    P = \begin{bmatrix}
    p_{11} & 0\\
    0 & p_{22}
    \end{bmatrix};
    Z = \begin{bmatrix}
    z_{11} & z_{12}\\
    z_{21} & z_{22}
    \end{bmatrix};
    W_0 = \begin{bmatrix}
    1 & 1\\
    1 & 1
    \end{bmatrix}.
\end{equation}
In this case, we have
\begin{equation}
    - {\left( {Z - {W_0}} \right)^T}P = 
    \begin{bmatrix}
    -p_{11}\left(z_{11}-1 \right) & 
    -p_{22}\left(z_{21}-1 \right)\\
    -p_{11}\left(z_{12}-1 \right) & 
    -p_{22}\left(z_{22}-1 \right)\end{bmatrix}.
\end{equation}
When $p_{ii}$ are small, the gradients backpropagated to update the remover’s parameters are also small, leaving the attacker hard to update the remover's gradient. Notably, the two-dimensional example can be easily generalized to higher-dimensional real-world situations.

==> sec_abandoned/5_experiment.tex <==

\section{Experiment}

\begin{figure*}[!ht]
    \centering
    % first line
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/derain_l1_various_m.png}
        \caption{L1 loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/derain_l2_various_m.png}
        \caption{L2 loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/derain_l2_consist_various_m.png}
        \caption{L2 and consistent losses}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/derain_no_defense.png}
        \caption{L2 loss with no defense}
    \end{subfigure}
    
    % second line
    \vspace{0.5cm} % 行间距
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/style_l1_various_m.png}
        \caption{L1 loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/style_l2_various_m.png}
        \caption{L2 loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/style_l2_consist_various_m.png}
        \caption{L2 and consistent losses}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/style_no_defense.png}
        \caption{L2 loss with no defense}
    \end{subfigure}
    
    \caption{Demonstration of the convergence behavior of various removal loss functions from the attacker's perspective. The first three columns display results with the proposed defense across different magnitudes of diagonal elements in the positive definite matrix $P$. The last column shows results without the proposed defense. The first row presents results for the deraining task, while the second row includes results for the style transfer task.}
    \label{fig:convergence_various_losses}
\end{figure*}
\label{sec:experiment}
In this section, we validate our proposed DGS against the gradient-based watermark removal attack through comprehensive experiments and ablation studies. We aim to defend the victim model described in \cite{zhang2021deep, zhang2024robust}. Notably, \cite{zhang2024robust} is an extended version of \cite{zhang2021deep}, addressing the vulnerabilities of their watermarking scheme to image augmentation attacks, despite sharing the same watermark encoding and decoding framework. In our experiments, we treat them as a single victim model, as image augmentation attacks are not considered and the core implementation is based on the open-source code from \cite{zhang2021deep}. In addition, Box-free model watermarking can be applied to models across various tasks. For consistency with the victim model, we select image processing models focused on deraining and style transfer as the underlying tasks in our experiments.

\subsection{Experimental Settings}
\subsubsection{Datasets}
For both deraining and style transfer tasks, we use the PASCAL VOC dataset \cite{everingham2010pascal} with different data splits. For image deraining, these data are denoted as $X$ in Figure \ref{fig:victim_architecture}. We uniformly split the $12,000$ training images into two equal parts, each containing $6,000$ images for victim model training and remover training. Rainy images, referred to as $X_0$, are generated using the algorithm in \cite{zhang2018density}. For style transfer, the PASCAL VOC data are treated as $X_0$ and similarly divided for victim and remover training. The style transfer algorithm from \cite{li2018learning} is employed to generate $X$. Additionally, to reduce computational complexity, we resize all images in datasets to $256 \times 256$ grayscale images.

\subsubsection{Metrics}
In our experiment, we use peak signal-to-noise ratio (PSNR) and multi-scale structural similarity index (MS-SSIM) \cite{wang2003multiscale} to evaluate the similarity between two images. Additionally, we define the success rate of defense, $\text{SR}_\text{D}$, as the ratio of successfully defended images to the total number of defended images. Specifically, a defense is considered successful when the normalized correlation coefficient between $W$ and $Z$ exceeds $0.96$, even higher than the threshold set in \cite{zhang2021deep}.

\subsubsection{Implementation Details}
We strictly follow the model architecture, hyperparameters and training process of victim model in \cite{zhang2021deep}. The gradient-based remover is implemented using a UNet architecture \cite{ronneberger2015u}. Both models are trained from scratch for 100 epochs using the Adam optimizer, with an initial learning rate of $0.0002$. Weighting parameters $\alpha_1$, $\alpha_2$, $\beta_1$, and $\beta_2$ in (\ref{eq:loss_joint}) and (\ref{eq:loss_attacker}) are set equally $10,000$. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/derain_l2_attacker_flip.png}
    \caption{Demonstration of the convergence behavior of $\ell_2$ removal loss in the deraining task from the defender's perspective. Various magnitudes of diagonal elements in matrix $P$ are tested.}
    \label{fig:attacker_flip}
\end{figure}
\subsection{Convergence of Removal loss}
\label{sec:convergence_r_loss}
We present the convergence results of the removal loss from two perspectives: 1) the attacker’s perspective and 2) the defender’s perspective.

From the attacker's view, the remover loss discussed in (\ref{eq:r_loss}) is rewritten as 
\begin{equation}
    \mathcal{L}^{A}_\text{Removal}  =  \|Z^{\ast} - W_0\|_2^2,
\end{equation}
since $Z = \mathbb{D}[\mathbb{R}(Y)] $ is inaccessible to the attacker. The convergence results for different loss functions used as the removal loss, with different scale of diagonal elements $p_{ii}$, to train the remover are presented in Figure \ref{fig:convergence_various_losses}. We evaluate commonly used $\ell_1$ and $\ell_2$ losses, as well as the consistent loss \cite{zhang2020model}, defined as
\begin{equation}
    \mathcal{L}_\text{C} = \|Z_{1:\left(N/2 \right)} - Z_{\left(1+N/2 \right):N}\|_2^2,
\end{equation}
where $Z_{1:\left(N/2 \right)}$ and $Z_{\left(1 + N/2 \right):N}$ represent the first and second halves of the batch of $Z$, respectively, and $N$ is the batch size.
The fidelity loss is consistently the $\ell_2$-norm loss function. The results for deraining and style transfer tasks are presented in the first and second rows, respectively. For both tasks, when no defense is employed, the magnitudes of all losses are on the order of $10^{-3}$. The $\ell_1$ loss converges around $0.2 \times 10^{-3}$, while using $\ell_2$ loss and $\ell_2$ plus consistent loss leads to convergence near zero. It is noted that the use of the consistent loss leads to a smoother convergence curve. In contrast, the magnitudes of all losses increase to the order of $10^{-1}$ when DGS is utilized, representing an over 100-fold increase. Furthermore, the convergence trend observed by the attacker may serve as a sleight of hand, obscuring the existence of defenses, as there is no explicit increase in loss from the attacker's perspective.

% Specifically, matrix P in (\ref{eq:ultimate_trans}) is square and positive definite, predefined as follows:
% \begin{equation}
% \label{matrix_p}
%     \begin{bmatrix}
% p_{11} & 0 & \cdots & 0 \\
% 0 & p_{22} & \cdots & 0 \\
% \vdots & \vdots & \ddots & \vdots \\
% 0 & 0 & \cdots & p_{nn}
% \end{bmatrix},
% \end{equation}
% where $n$ is the dimension of $Z$ and $p_{ii} > 0$, $i$ from $1$ to $n$. We randomly sample $p_{ii}$ in three ranges, $10^{-2}$ to $10{-1}$, $10{-3}$ to $10^{-2}$, and $10{-5}$ to $10^{-4}$, noting that for both deraining and style transfer tasks, smaller values of $p_{ii}$ provide a smoother convergence curve and results in the highest convergence magnitude across all adopted losses. We offer the following analysis: Based on (\ref{eq:z_inverse}), a 2-dimensional example can be expressed as
% \begin{equation}
%     P = \begin{bmatrix}
%     p_{11} & 0\\
%     0 & p_{22}
%     \end{bmatrix};
%     Z = \begin{bmatrix}
%     z_{11} & z_{12}\\
%     z_{21} & z_{22}
%     \end{bmatrix};
%     W_0 = \begin{bmatrix}
%     1 & 1\\
%     1 & 1
%     \end{bmatrix}.
% \end{equation}
% In this case, we have
% \begin{equation}
%     - {\left( {Z - {W_0}} \right)^T}P = 
%     \begin{bmatrix}
%     -p_{11}\left(z_{11}-1 \right) & 
%     -p_{22}\left(z_{21}-1 \right)\\
%     -p_{11}\left(z_{12}-1 \right) & 
%     -p_{22}\left(z_{22}-1 \right)\end{bmatrix}.
% \end{equation}
% When $p_{ii}$ are small, the gradients backpropagated to update the remover’s parameters are also small, which explains the observed smoother convergence curve and higher convergence magnitude.

From the defender's view, the remover loss remains the same as (\ref{eq:r_loss}). The curves of $\ell_2$ removal loss for the deraining tasks with different magnitudes of $p_{ii}$ are presented in Figure \ref{fig:attacker_flip}. Our DGS increases the gradient and converges around $1.3 \times 10^{-1}$ with varying speeds depending on the magnitude of $p_{ii}$ employed.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/effectiveness_no_defense.pdf}
    \caption{Demonstration of gradient-based attack against the victim model without defense. (a) Deraining task and (b) Style transfer task. Images are converted to grayscale to reduce computational complexity.}
    \label{fig:effectiveness_no_defense}
\end{figure}
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/effectiveness.pdf}
    \caption{Demonstration of gradient-based attack on the victim model with the proposed DGS under different losses. The first three rows show the deraining task, while the remaining rows display the style transfer task. The attacker applies $\ell_1$ loss in (a) and (d), $\ell_2$ loss in (b) and (e), and a combination of $\ell_2$ and consistent losses in (c) and (f). Images are converted to grayscale to reduce computational complexity.}
    \label{fig:effectiveness}
\end{figure}


\subsection{Effectiveness}
\label{sec:effectiveness}
The visible results of our method are shown in Figure \ref{fig:effectiveness_no_defense} (without DGS) and Figure \ref{fig:effectiveness} (with DGS), demonstrating the effectiveness of the proposed defense. In both the deraining and style transfer tasks, when lack of defense, the gradient-based removal attack successfully removes the watermark from $Y$, producing an all-white image at $Z$. In contrast, DGS prevents $Z$ from converging to an all-white image across various attacker loss functions ((a) and (d) use $\ell_1$ loss, (b) and (e) use $\ell_2$ loss, and (c) and (f) use a combination of $\ell_2$ and consistent losses), as shown the extracted watermark $Z$ ensembles the embedded $W$. Additionally, DGS preserves decoder output image quality, with $Z^{\ast}$ closely matching $\mathbb{D}\left(Y\right)$, allowing benign users to use the system normally while concealing the gradient shield from the attacker.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/robustness_attacker_flip.pdf}
    \caption{Demonstration of robustness of our proposed DGS at Vulnerability Level 3, with $p_{ii}$ randomly sampled in the range of (a) $10^{-5}$ to $10^{-4}$, (b) $10^{-6}$ to $10^{-5}$, (c) $10^{-7}$ to $10^{-6}$, and (d) $10^{-8}$ to $10^{-7}$.}
    \label{fig:robustness_attacker_flip}
\end{figure}

\subsection{Robustness}
\label{sec:robustness}
We evaluate the robustness of our proposed DGS under the Vulnerability Level 2 and 3 discussed in Section \ref{sec:p_choice}.

For Level 2, plausible ways to bypass the defense include operations on $Z^{\ast}$, such as applying JPEG compression, Gaussian noise, and lattice attacks \cite{liu2023erase}. The lattice attack, in particular, replaces pixels with random values at fixed intervals. Results for each attack are presented in Table \ref{tab:JPEG_compression}, Table \ref{tab:Gaussian_noise}, and Table \ref{tab:lattice_attack}, respectively. SNR and MS-SSIM are used to measure the similarity between the original and attacked $Z^{\ast}$. Our results show that DGS is highly robust against these attacks, with defense success rates $1.00$, except for a performance drop in the style transfer task at a noise level of 0 dB. These attacks can be modeled as introducing an interference term $F$ into
(\ref{eq:ultimate_trans}) as
\begin{equation}
    \label{eq:interfered_shield}
    Z^{\ast}_{\text{Interf}} = -PZ + (P+I)W + F,
\end{equation}
where $F$ is independent of $Z$. Substituting $Z^{\ast}_{\text{Interf}}$ for $Z^{\ast}$ in (\ref{eq:poison_gradient}) yields
\begin{equation}
    2{\left( {Z^{\ast}_{\text{Interf}} - {W_0}} \right)^T}\frac{{\partial Z^\ast_{\text{Interf}}}}{{\partial \mathbb{R}(Y)}},
\end{equation}
which simplifies to
\begin{equation}
    -2{\left[ {Z - \left({W_0} - F \right)} \right]^T}P\frac{{\partial Z}}{{\partial \mathbb{R}(Y)}}.
\end{equation}
These attacks are equivalent to forcing the model to converge the output toward the target value $W_0 - F$ while moving in the opposite direction of the gradient. As a result, they cannot neutralize our defense. Additionally, DGS proves insensitive to data distribution, as shown by the near-symmetry in the values of two tasks across all three tables.

For Level 3, we assume the attacker has full knowledge of the DGS mechanism, enabling them to directly flip the sign as described in (\ref{eq:params_update}) and (\ref{eq:flip_params_update}). Despite this, as detailed in Section \ref{sec:p_choice}, small $p_{ii}$ can help. We show the visible results in Figure \ref{fig:robustness_attacker_flip}, with $p_{ii}$ set within the ranges of $10^{-5}$ to $10^{-4}$, $10^{-6}$ to $10^{-5}$, $10^{-7}$ to $10^{-6}$, and $10^{-8}$ to $10^{-7}$. We notice that when $p_{ii}$ is randomly sampled from values between $10^{-7}$ to $10^{-6}$ or lower, DGS remains robust to gradient-based removal attacks.

\begin{table}[!t]
  \centering
  \caption{Robustness results for proposed DGS against JPEG compression, where $10^{-5}<p_{ii}<10^{-4}$, PSNR is in dB, $0< \text{MS-SSIM} <1$, and $0<\text{SR}_{\text{D}}<1$.}
  % \vspace*{-9pt}
  \setlength{\tabcolsep}{1pt}
  \label{tab:JPEG_compression}
  \begin{tabular}{c|ccc|ccc}
  \hline
  \hline
  \multirow{2}{*}{Factor} & \multicolumn{3}{c}{Deraining} & \multicolumn{3}{c}{Style Transfer} \\
  \cline{2-7}
  & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & $\text{SR}_{\text{D}}\uparrow$ & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & $\text{SR}_{\text{D}}\uparrow$  \\
  \hline
  $10\%$ & $28.5748$ & $0.9672$ & $1.00$ & $28.5776$ & $0.9673$ & $1.00$ \\ 
  $20\%$ & $30.8380$ & $0.9855$ & $1.00$ & $30.8364$ & $0.9855$ & $1.00$ \\ 
  $30\%$ & $32.0850$ & $0.9902$ & $1.00$ & $32.0845$ & $0.9902$ & $1.00$ \\ 
  $40\%$ & $33.0321$ & $0.9927$ & $1.00$ & $33.0278$ & $0.9927$ & $1.00$ \\ 
  \hline
  \hline
  \end{tabular}
  \end{table}

\begin{table}[!t]
  \centering
  \caption{Robustness results for proposed DGS against Gaussion white noise adding, where $10^{-5}<p_{ii}<10^{-4}$, noise level and PSNR are in dB, $0< \text{MS-SSIM} <1$, and $0<\text{SR}_{\text{D}}<1$.}
  % \vspace*{-9pt}
  \setlength{\tabcolsep}{1pt}
  \label{tab:Gaussian_noise}
  \begin{tabular}{c|ccc|ccc}
  \hline
  \hline
  \multirow{2}{*}{\begin{tabular}{@{}c@{}} Noise \\ Level \end{tabular}} & \multicolumn{3}{c}{Deraining} & \multicolumn{3}{c}{Style Transfer} \\
  \cline{2-7}
  & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & $\text{SR}_{\text{D}}\uparrow$ & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & $\text{SR}_{\text{D}}\uparrow$  \\
  \hline
  $0$ & $1.7791$ & $0.3042$ & $1.00$ & $1.7768$ & $0.3041$ & $0.58$ \\ 
  $10$ & $11.7799$ & $0.5613$ & $1.00$ & $11.7809$ & $0.5612$ & $1.00$ \\ 
  $20$ & $21.7774$ & $0.8022$ & $1.00$ & $21.7801$ & $0.8022$ & $1.00$ \\ 
  $30$ & $31.7781$ & $0.9573$ & $1.00$ & $31.7784$ & $0.9573$ & $1.00$ \\ 
  \hline
  \hline
  \end{tabular}
  \end{table}

\begin{table}[!t]
  \centering
  \caption{Robustness results for proposed DGS against lattice attack, where $10^{-5}<p_{ii}<10^{-4}$, PSNR is in dB, $0< \text{MS-SSIM} <1$, and $0<\text{SR}_{\text{D}}<1$.}
  % \vspace*{-9pt}
  \setlength{\tabcolsep}{1pt}
  \label{tab:lattice_attack}
  \begin{tabular}{c|ccc|ccc}
  \hline
  \hline
  \multirow{2}{*}{Interval} & \multicolumn{3}{c}{Deraining} & \multicolumn{3}{c}{Style Transfer} \\
  \cline{2-7}
  & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & $\text{SR}_{\text{D}}\uparrow$ & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & $\text{SR}_{\text{D}}\uparrow$  \\
  \hline
  $2$ & $12.3766$ & $0.6391$ & $1.00$ & $12.3766$ & $0.6391$ & $1.00$ \\ 
  $6$ & $21.9368$ & $0.8275$ & $1.00$ & $21.9370$ & $0.8275$ & $1.00$ \\ 
  $11$ & $26.8371$ & $0.9263$ & $1.00$ & $26.8373$ & $0.9263$ & $1.00$ \\ 
  $16$ & $30.6777$ & $0.9655$ & $1.00$ & $30.6777$ & $0.9655$ & $1.00$ \\ 
  \hline
  \hline
  \end{tabular}
  \end{table}
% \subsection{}
% For generalization, we consider mean absolute error (MAE, also called L1 loss) is used by attacker, turning (\ref{eq:original_gradient}) into
% \begin{equation}
%     \frac{{\partial {\mathcal{L}_{\text{R}}}}}{{\partial Y}} = |Z - W_0|\frac{\partial Z}{{\partial Y}},\label{eq:general_original_gradient}
% \end{equation}
% and (\ref{eq:poison_gradient}) into
% \begin{equation}
%     \frac{{\partial {\mathcal{L}_{\text{R}}}}}{{\partial Y}} = - |Z^\ast - W_0|P\frac{\partial Z}{{\partial Y}},\label{eq:general_poison_gradient}
% \end{equation}


\subsection{Ablation Study}
\label{sec:ablation}
% \subsection{Necessity of Matrix $P$}

In the derivation of (\ref{eq:ultimate_trans}), positive definite matrix $P$ can be viewed as a generalization of a positive scalar. While it does not fully redirect the gradient by $180$ degrees, it introduces some flexibility for the defender. However, the necessity of this additional computational overhead is questionable when only Vulnerability Level 1 and 2 are considered. To explore this, we remove matrix $P$ (or set it to the identity matrix) in (\ref{eq:ultimate_trans}), resulting in
\begin{equation}
    Z^\ast = -Z + 2W,
\end{equation}
which fully reorients the gradient. The results of convergence when the attacker employs different losses function are presented in Figure \ref{fig:no_P_plot}. When compared to the curves in Figure \ref{fig:convergence_various_losses}, we observe that using a matrix $P$ leads to higher convergence values and faster convergence speed. Moreover, matrix $P$ is a sparse matrix, as only the diagonal elements are non-zero, leading to tolerable computational overhead since GPUs excel at computing sparse matrix multiplications. 

\label{sec:ablation_study}
\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/no_P_plot_derain.png} 
        \caption{Deraining}
        \label{fig:no_P_plot_derain}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/no_P_plot_style.png} 
        \caption{Style transfer}
        \label{fig:no_P_plot_style}
    \end{subfigure}
    \caption{Ablation study on the necessity of Matrix $P$. Convergence results of $\ell_1$ loss, $\ell_2$ loss, and the combination of $\ell_2$ and consistent losses are demonstrated for both deraining and style transfer tasks.}
    \label{fig:no_P_plot}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figure/l2_solo.png}
%     \caption{Ablation study on the impact of combining removal and fidelity losses. Only the $\ell_2$ loss is used to train the gradient-based remover.}
%     \label{fig:l2_solo}
% \end{figure}
% \subsection{Effect of Losses Combination}
% We note that although DGS reorients the gradient from malicious attacks, as discussed in Section \ref{sec:gr}, the experimental results in Figures \ref{fig:convergence_various_losses} and Figure \ref{fig:no_P_plot} show an increase in convergence of the loss, rather than an increase in the loss itself. A plausible hypothesis is that the combination of removal loss and fidelity loss in (\ref{eq:loss_attacker}) strikes a balance, leading to an elevated convergence level. To verify this, we remove the fidelity loss during the training of the gradient-based remover and use only the $\ell_2$-norm loss as the removal loss with $10^{-2} < p_{ii} < 10^{-1}$ to observe the convergence process. The results for deraining and style transfer tasks are shown in Figure \ref{fig:l2_solo}. It can be seen that the increased convergence level persists without a corresponding increase in loss value. Although this is a desirable property since the attacker cannot flip the sign during remover parameters (e.g., $w_i$) updating like turning
% \begin{equation}
%     w_i - \frac{\partial \mathcal{L}_{\text{Removal}}}{\partial w_i}
% \end{equation}
% into
% \begin{equation}
%     w_i + \frac{\partial \mathcal{L}_{\text{Removal}}}{\partial w_i}
% \end{equation}
% to bypass DGS, the underlying mechanism requires further investigation in future work.

\subsection{Limitation}
\label{sec:limitation}
The attacker can bypass DGS if $Z$ can be recovered from (\ref{eq:ultimate_trans}), i.e.,
\begin{equation}
    Z = - P^{-1}Z^{\ast} + \left(I + P^{-1}\right)W .
\end{equation}
However, The attacker lacks knowledge of both $P$ and $W$. As discussed in Section \ref{sec:ablation}, while matrix $P$ influences the convergence value and speed but does not significantly affect defense's success rate. Thus, the attacker can attempt to remove the positive definite matrix $P^{-1}$, aiming to re-reorient the gradient. Only if $W$ is revealed to the attacker, gradient can be re-reoriented by
\begin{equation}
    \Tilde{Z} = - Z^{\ast} + 2W.
\end{equation}
In (\ref{eq:z_quality}), DGS assumes $Z^\ast$, which the attacker can obtain from the output of $\mathbb{D}$'s API, resembles $W$. In this case, it is at risk of $W$ leakage, compromising the defense's efficacy. Therefore, an improved version of DGS that better conceals the information of $W$ requires further investigation in the future.



\section{Conclusion}
\label{sec:conclusion}


==> sec_abandoned/6_ablation_study.tex <==
\section{Ablation Study}
\label{sec:ablation}
% \subsection{Necessity of Matrix $P$}

In the derivation of (\ref{eq:ultimate_trans}), positive definite matrix $P$ can be viewed as a generalization of a positive scalar. While it does not fully redirect the gradient by $180$ degrees, it introduces some flexibility for the defender. However, the necessity of this additional computational overhead is questionable when only Vulnerability Level 1 and 2 are considered. To explore this, we remove matrix $P$ (or set it to the identity matrix) in (\ref{eq:ultimate_trans}), resulting in
\begin{equation}
    Z^\ast = -Z + 2W,
\end{equation}
which fully reorients the gradient. The results of convergence when the attacker employs different losses function are presented in Figure \ref{fig:no_P_plot}. When compared to the curves in Figure \ref{fig:convergence_various_losses}, we observe that using a matrix $P$ leads to higher convergence values and faster convergence speed. Moreover, matrix $P$ is a sparse matrix, as only the diagonal elements are non-zero, leading to tolerable computational overhead since GPUs excel at computing sparse matrix multiplications. 

\label{sec:ablation_study}
\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/no_P_plot_derain.png} 
        \caption{Deraining}
        \label{fig:no_P_plot_derain}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/no_P_plot_style.png} 
        \caption{Style transfer}
        \label{fig:no_P_plot_style}
    \end{subfigure}
    \caption{Ablation study on the necessity of Matrix $P$. Convergence results of $\ell_1$ loss, $\ell_2$ loss, and the combination of $\ell_2$ and consistent losses are demonstrated for both deraining and style transfer tasks.}
    \label{fig:no_P_plot}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figure/l2_solo.png}
%     \caption{Ablation study on the impact of combining removal and fidelity losses. Only the $\ell_2$ loss is used to train the gradient-based remover.}
%     \label{fig:l2_solo}
% \end{figure}
% \subsection{Effect of Losses Combination}
% We note that although DGS reorients the gradient from malicious attacks, as discussed in Section \ref{sec:gr}, the experimental results in Figures \ref{fig:convergence_various_losses} and Figure \ref{fig:no_P_plot} show an increase in convergence of the loss, rather than an increase in the loss itself. A plausible hypothesis is that the combination of removal loss and fidelity loss in (\ref{eq:loss_attacker}) strikes a balance, leading to an elevated convergence level. To verify this, we remove the fidelity loss during the training of the gradient-based remover and use only the $\ell_2$-norm loss as the removal loss with $10^{-2} < p_{ii} < 10^{-1}$ to observe the convergence process. The results for deraining and style transfer tasks are shown in Figure \ref{fig:l2_solo}. It can be seen that the increased convergence level persists without a corresponding increase in loss value. Although this is a desirable property since the attacker cannot flip the sign during remover parameters (e.g., $w_i$) updating like turning
% \begin{equation}
%     w_i - \frac{\partial \mathcal{L}_{\text{Removal}}}{\partial w_i}
% \end{equation}
% into
% \begin{equation}
%     w_i + \frac{\partial \mathcal{L}_{\text{Removal}}}{\partial w_i}
% \end{equation}
% to bypass DGS, the underlying mechanism requires further investigation in future work.

\section{Limitation}
\label{sec:limitation}
The attacker can bypass DGS if $Z$ can be recovered from (\ref{eq:ultimate_trans}), i.e.,
\begin{equation}
    Z = - P^{-1}Z^{\ast} + \left(I + P^{-1}\right)W .
\end{equation}
However, The attacker lacks knowledge of both $P$ and $W$. As discussed in Section \ref{sec:ablation}, while matrix $P$ influences the convergence value and speed but does not significantly affect defense's success rate. Thus, the attacker can attempt to remove the positive definite matrix $P^{-1}$, aiming to re-reorient the gradient. Only if $W$ is revealed to the attacker, gradient can be re-reoriented by
\begin{equation}
    \Tilde{Z} = - Z^{\ast} + 2W.
\end{equation}
In (\ref{eq:z_quality}), DGS assumes $Z^\ast$, which the attacker can obtain from the output of $\mathbb{D}$'s API, resembles $W$. In this case, it is at risk of $W$ leakage, compromising the defense's efficacy. Therefore, an improved version of DGS that better conceals the information of $W$ requires further investigation in the future.

\section{Conclusion}
\label{sec:conclusion}

